Empirical Bayes approach to Truth Discovery problems

When aggregating information from conflicting sources, one's goal is to find the truth. Most real-value \emph{truth discovery} (TD) algorithms try to achieve this goal by estimating the competence of each source and then aggregating the conflicting information by weighing each source's answer proportionally to her competence. However, each of those algorithms requires more than a single source for such estimation and usually does not consider different estimation methods other than a weighted mean. Therefore, in this work we formulate, prove, and empirically test the conditions for an Empirical Bayes Estimator (EBE) to dominate the weighted mean aggregation. Our main result demonstrates that EBE, under mild conditions, can be used as a second step of any TD algorithm in order to reduce the expected error.

==> forThesis.tex <==
\subsection{EBE advantage analysis in Bayes Risk}
As the variance of the prior distribution grows, the visible gap between the EBE to BLUE is getting narrower; as the workers' variance grows, the same gap is getting wider. Following similar notions as Efron and Morris in \cite{10.2307/2284155}, we try to give some intuition.
For convenience we assume the settings as in \ref{stein_estimator}: let $\mu_j\sim \mathcal{N}(0, \sigma_0^2)$, we assume $\mu_0$ is known and equal to 0. Consequently, the posterior distribution as presented at (\ref{posterior}) is:
$$\mu_j|X_j \sim \mathcal{N}(\frac{X_j\sigma_0^2}{\sigma_0^2 + \bar{\sigma}^2}, \frac{\bar{\sigma}^2\sigma_0^2}{\sigma_0^2 + \bar{\sigma}^2})$$
Where $X_j|\mu_j\sim \mathcal{N}(\mu_j, \bar{\sigma}^2)$. The BLUE estimator is just the observed $X$. Using the results from \ref{posterior} the BLUE risk $\mathcal{R}_{\mu, \sigma}(\delta_B) = E_{\mu, \sigma}[X_j - \mu_j]^2 = \bar{\sigma}^2$ and the EBE risk $\mathcal{R}_{\mu, \sigma}(E_{\mu, \sigma}(\mu_j|X_j), \mu_j) = Var_{\mu, \sigma}(\mu_j|X_j) = \frac{\bar{\sigma}^2\sigma_0^2}{\sigma_0^2 + \bar{\sigma}^2}$ subtracting the one result from the other we get the following:
\begin{equation*}\label{RiskDiff}
    \mathcal{R}_{\mu, \sigma}(\delta_B) - \mathcal{R}_{\mu, \sigma}(\delta_{EBE}) = \frac{\bar{\sigma}^4}{\sigma_0^2 + \bar{\sigma}^2}
\end{equation*}
Larger prior's variance $\sigma_0^2$, means a smaller advantage EBE has over BLUE but larger $\bar{\sigma}^2$ means the opposite.

==> old_tables.tex <==
\begin{table}
 %\begin{minipage}{.5\linewidth}
 \begin{scriptsize}
 \begin{center}
  $ \begin{array}{|c|c|c|c|c|c|c|c|c|c|}\hline  
 ALG / DS & \Delta &BUILD & TRI1 & TRI2 & EMO1 & EMO2 & EMO3 & EMO4\\ \hline
 \multirow{2}{2em}{
 UA
 }                                   &\Delta_{EBE} &
 \tnum{-1.8E-02} & \tnum{-6.3E-3} & \tnum{-7.5E-03} & \best{\tnum{1.5E-02}} & \tnum{8.8E-03} & \best{\tnum{1.6E-02}} & \tnum{7.3E-03} \\
                                    & \Delta_{Stein} &
 \tnum{8.5E-03} & \tnum{2.1E-2} & \tnum{1.1E-03} & \tnum{8.8E-03} & \tnum{8.5E-04} & \tnum{1.3E-02} & \tnum{8E-04}\\ \hline
 \multirow{3}{2em}{
 DTD
 }&
                                     \Delta_{EBE} &
 \tnum{-1.8E-02} & \tnum{-6.3E-03} & \tnum{-7.5E-03} & \tnum{1.5E-02} & \best{\tnum{8.7E-03}} & \tnum{1.6E-02} & \best{\tnum{7.2E-03}}\\
                                   & \Delta_{Stein} &
 \tnum{8.7E-03} & \tnum{2.1E-03} & \tnum{1.1E-03} & \tnum{8.8E-03} & \tnum{8.1E-04} & \tnum{1.3E-02} & \tnum{7.4E-04}\\ 
                                   & \Delta_{Iter} &
 \tnum{1.8E+00} & \tnum{1.3E+00} & \tnum{1.3E+00} & \tnum{9.3E-02} & \tnum{-3.1E-02} & \tnum{-1E-01} & \tnum{-5.5E-02}\\ \hline
  \multirow{3}{2em}{
 PTD
 }
                                      &\Delta_{EBE} &
 \tnum{3.3E-03} & \tnum{-3.8E-03} & \tnum{-5.1E-03} & \tnum{4.9E-03} & \tnum{-3.2E-03} & \tnum{8.1E-03} & \tnum{1.2E-03}\\
                                    & \Delta_{Stein} &
 \tnum{6.1E-04} & \tnum{2.3E-03} & \tnum{7.8E-04} & \tnum{-3.9E-03} & \tnum{-1.3E-02} & \tnum{4.0E-03} & \tnum{-6.3E-03}\\
                                    & \Delta_{Iter} &
 \tnum{-1.5E+00} & \tnum{-8.5E-02} & \tnum{1.8E-02} & \tnum{-2.6E-04} & \tnum{3.6E-03} & \tnum{7.6E-03} & \tnum{1.9E-03}\\ \hline
 \multirow{3}{2em}{
 CRH
 }
                                    & \Delta_{EBE} &
 \tnum{-1E-02} & \tnum{-3.6E-02} & \tnum{-4.5E-03} & \tnum{4.6E-03} & \tnum{-2.1E-03} & \tnum{7.8E-03} & \tnum{1.6E-03}\\
                                   & \Delta_{Stein} &
 \tnum{2.4E-03} & \best{\tnum{2.3E-03}} & \best{\tnum{6.9E-04}} & \tnum{-2.8E-03} & \tnum{-1.1E-02} & \tnum{4.3E-03} & \tnum{-5.1E-03}\\
                                    & \Delta_{Iter} &
 \tnum{-7.7E-01} & \tnum{-3.3E-02} & \tnum{-7.2E-03} & \tnum{-1.9E-03} & \tnum{-5.9E-03} & \tnum{-2.3E-03} & \tnum{-2.9E-03}\\ \hline
 \multirow{3}{2em}{
 CATD
 }                                &\Delta_{EBE} &
 \tnum{-6.3E-05} & \tnum{-2.5E-03} & \tnum{-4.5E-05} & \tnum{5.6E-05} & \tnum{2.9E-04} & \tnum{2.4E-04} & \tnum{3.8E-05} \\
                                & \Delta_{Stein} &
 \tnum{9.2E-05} & \tnum{2E-03} & \tnum{9E-06} & \tnum{-1.2E-04} & \tnum{2E-04} & \tnum{2.3E-04} & \tnum{-1.2E-04}\\
                                    & \Delta_{Iter} &
 \tnum{-1.1E+02} & \tnum{-1.2E+0} & \tnum{-1.7E+00} & \tnum{-1.1E+00} & \tnum{-7E-01} & \tnum{-2.3E-03} & \tnum{-1.8E+00}\\ \hline
 \multirow{3}{2em}{
 GTM
}                                  &\Delta_{EBE} &
 \tnum{-1.4E-02} & \tnum{-6E-03} & \tnum{-7.3E-03} & \tnum{1.1E-02} & \tnum{2.6E-03} & \tnum{1.3E-02} & \tnum{5.3E-03}\\
                                  & \Delta_{Stein} &
 \best{\tnum{5.4E-03}} & \tnum{2.3E-03} & \tnum{1.1E-03} & \tnum{1.9E-03} & \tnum{-8.5E-03} & \tnum{8.4E-03} & \tnum{-3.0E-03}\\ 
                                                            & \Delta_{Iter} &
 \tnum{-3.3E-07} & \tnum{-9.1E-12} & \tnum{1.3E-09} & \tnum{0E+00} & \tnum{0E+00} & \tnum{0E+00} & \tnum{0E+00}\\ \hline
 \multirow{3}{2em}{
 KDEm
 }                                                                                                                           &\Delta_{EBE} &
 \tnum{-1.3E-02} & \tnum{-2E-03} & \tnum{-6.9E-03} & \tnum{-2.9E-02} & \tnum{-3.3E-03} & \tnum{-9.9E-03} & \tnum{-1.2E-02}\\
                                 & \Delta_{Stein} &
 \tnum{1.5E-03} & \tnum{3E-03} & \tnum{1.1E-03} & \tnum{-6.2E-02} & \tnum{-7.1E-02} & \tnum{-2.1E-02} & \tnum{-4.1E-02}\\ 
                                  & \Delta_{Iter} &
 \tnum{0} & \tnum{0} & \tnum{0} & \tnum{0} & \tnum{0} & \tnum{0} & \tnum{0}\\ 
 \hline
%OA(S)&&8.31&-0.40&3.80&2.13&0.01\\

    \end{array}$
    \end{center}
    \end{scriptsize}\vspace{-2mm}
    \caption{Results of real-world datasets, columns are datasets and rows are algorithms, each value is calculated over 1,000 samples of 5 workers who answered 10 questions, bold and underlined has the lowest MSE for a dataset e.g 14 iterations of GTM and then applying Stein has the lowest MSE for the Buildings data set.}
    
    \label{results_real}
    \end{table}

 \begin{table}
 %\begin{minipage}{.5\linewidth}
 \begin{scriptsize}
 \begin{center}
  $ \begin{array}{|c|c|c|c|c|c|}\hline  
 ALG / DS & \Delta & GT_j=0, X_{ij}\sim N(GT_j,\sigma_i^2) & GT_j\sim N(0,2),X_{ij}(GT_j,\sigma_i^2) & GT \sim N(2,2), X_{ij} \sim (GT_j,\sigma_i^2)\\ \hline
 \multirow{2}{2em}{
Mean
 }                                   &\Delta_{EBE} &
 \tnum{5.1E-02} & \tnum{3.1E-03} & \tnum{2.9E-03}  \\
                                    & \Delta_{Stein} &
 \tnum{5.8E-02} & \tnum{3.5E-03} & \tnum{1.4E-03} \\ \hline
 \multirow{3}{2em}{
 DTD
 }&
                                     \Delta_{EBE} &
 \tnum{5.1E-02} & \tnum{3.1E-03} & \tnum{2.9E-03}\\
                                   & \Delta_{Stein} &
 \tnum{5.8E-02} & \tnum{3.5E-03} & \tnum{1.4E-03}\\ 
                                   & \Delta_{Iter} &
 \tnum{0E+00} & \tnum{0E+00} & \tnum{0E+00}\\ \hline
  \multirow{3}{2em}{
 PTD
 }
                                      &\Delta_{EBE} &
 \tnum{4E-02} & \tnum{1.9E-03} & \tnum{1.7E-03} \\
                                    & \Delta_{Stein} &
 \tnum{4.6E-02} & \tnum{2.2E-03} & \tnum{9E-04} \\
                                    & \Delta_{Iter} &
 \tnum{-1.2E-06} & \tnum{7.6E-07} & \tnum{-1E-05}\\ \hline
 \multirow{3}{2em}{
 CRH
 }
                                    & \Delta_{EBE} &
 \tnum{3.6E-02} & \tnum{1.7E-03} & \best{\tnum{1.5E-03}} \\
                                   & \Delta_{Stein} &
 \best{\tnum{4.1E-02}} & \best{\tnum{1.9E-03}} & \tnum{6.9E-04}\\
                                    & \Delta_{Iter} &
 \tnum{1.1E-07} & \tnum{1.7E-07} & \tnum{-7.2E-03}\\ \hline
 \multirow{3}{2em}{
 CATD
 }                                &\Delta_{EBE} &
 \tnum{1.4E-03} & \tnum{1.2E-04} & \tnum{1.5E-03}  \\
                                & \Delta_{Stein} &
 \tnum{1.6E-03} & \tnum{1.3E-04} & \tnum{7.7E-04} \\
                                    & \Delta_{Iter} &
 \tnum{-2.3E-03} & \tnum{-2.7E-03} & \tnum{9.5E-08} \\ \hline
 \multirow{3}{2em}{
 GTM
}                                  &\Delta_{EBE} &
 \tnum{4.9E-02} & \tnum{2.6E-03} & \tnum{2.4E-03} \\
                                  & \Delta_{Stein} &
 \tnum{5.6E-02} & \tnum{2.9E-03} & \tnum{1.2E-03}\\ 
                                                            & \Delta_{Iter} &
 \tnum{0E+00} & \tnum{0E+00} & \tnum{0E+00}\\ \hline
 \multirow{3}{2em}{
 KDEm
 }                                                                                                                           &\Delta_{EBE} &
 \tnum{5E-02} & \tnum{4.1E-03} & \tnum{3.8E-03} \\
                                 & \Delta_{Stein} &
 \tnum{5.7E-02} & \tnum{4.7E-03} & \tnum{2.1E-03} \\ 
                                  & \Delta_{Iter} &
 \tnum{0E+00} & \tnum{0E+00} & \tnum{0E+00} \\ 
 \hline
%OA(S)&&8.31&-0.40&3.80&2.13&0.01\\

    \end{array}$
    \end{center}
    \end{scriptsize}\vspace{-2mm}
    \caption{Results of synthetic datasets, columns are datasets and rows are algorithms, each value is calculated over 1,000 samples of 5 workers who answered 10 questions, each $\sigma_i^2 \sim N(1,.5)$ for all datasets. Bold and underlined has the lowest MSE for a dataset e.g 14 iterations of CRH and then applying EBE has the lowest MSE for the first column data set.}
    
    \label{results_syn}
    \end{table}
